An Approach to Model Checking of Multi-agent Data Analysis

The paper presents an approach to verification of a multi-agent data analysis algorithm. We base correct simulation of the multi-agent system by a finite integer model. For verification we use model checking tool SPIN. Protocols of agents are written in Promela language and properties of the multi-agent data analysis system are expressed in logic LTL. We run several experiments with SPIN and the model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{M. M. Bersani, D. Bresolin, L. Ferrucci and M. Mazzara (Eds.): \\
First Workshop on Logics and MODel-checking for self-* systems (MOD*)\\
EPTCS 168, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.168.3}{10.4204/EPTCS.168.3}}

